Towards Deep Attention in Graph Neural Networks: Problems and Remedies

Graph neural networks (GNNs) learn the representation of graph-structured data, and their expressiveness can be further enhanced by inferring node relations for propagation. Attention-based GNNs infer neighbor importance to manipulate the weight of its propagation. Despite their popularity, the discussion on deep graph attention and its unique challenges has been limited. In this work, we investigate some problematic phenomena related to deep graph attention, including vulnerability to over-smoothed features and smooth cumulative attention. Through theoretical and empirical analyses, we show that various attention-based GNNs suffer from these problems. Motivated by our findings, we propose AEROGNN, a novel GNN architecture designed for deep graph attention. AERO-GNN provably mitigates the proposed problems of deep graph attention, which is further empirically demonstrated with (a) its adaptive and less smooth attention functions and (b) higher performance at deep layers (up to 64). On 9 out of 12 node classification benchmarks, AERO-GNN outperforms the baseline GNNs, highlighting the advantages of deep graph attention. Our code is available at https://github.com/syleeheal/AERO-GNN.

==> Main-Text/031.define-T.tex <==
{A systematic understanding of graph attention, integrating edge and hop attention, would allow us to discuss various attention-based GNNs and their theoretical limitations within the same framework.}

\smallsection{Cumulative Attention.}
We have observed that edge and hop attention achieve the same goal (i.e., inferring the relational importance between node pairs), but from two different perspectives. 
Consequently, they both learn weights in which each node's features propagate to its neighbors.
This observation motivates us to integrate edge and hop attention under the same umbrella.
To this end, we propose a concept of \textit{cumulative attention matrix}, denoted by $T^{(k)}$, which intuitively represents attention between all node pairs within $k$ hops (or equivalently, at layer $k$) that considers both edge and hop attentions.

Formally, given any $k_{max}$, for each $0 \leq k \leq k_{max}$,
% \begin{equation}\label{eq:cumulative attention matrix}
% T^{(k)} = \Gamma^{(k)} \prod\nolimits_{l = 1}^k \mathcal{A}^{(\ell)},\forall k.
% \end{equation}
\begin{equation}\label{eq:cumulative attention matrix}
    T^{(k)} =  \Gamma^{(k)} \prod\nolimits_{\ell = k}^1 \mathcal{A}^{(\ell)},
\end{equation}
where $T^{(0)} = \Gamma^{(0)}$.\footnote{For FAGCN, $T^{(k)} = \Gamma^{(k)} \prod\nolimits_{\ell = k_{max}}^{k_{max} - k + 1} \mathcal{A}^{(\ell)}$. However, in our theoretical analyses, it is equivalent to Eq.~\eqref{eq:cumulative attention matrix} when $k_{max}$ is fixed.} 

% \smallsection{Cumulative Attention.}
% First, we establish a connection between edge attention and hop attention.
% We have observed that both edge attention and hop attention tackle essentially the same problem, i.e., inferring relational importance among nodes, but from two different perspectives. 
% Consequently, they both learn weights in which each node propagates to its neighbors.
% This observation motivates us to integrate edge and hop attention under the same umbrella using \textit{cumulative attention matrices} $T^{(k)}$'s, 
% which intuitively represent the attention between all the node pairs within $k$ hops, considering both edge and hop attention. 
% Formally, fix any $k_{max}$, and for each $0 \leq k \leq k_{max}$,
% % \begin{equation}\label{eq:cumulative attention matrix}
% % T^{(k)} = \Gamma^{(k)} \prod\nolimits_{l = 1}^k \mathcal{A}^{(\ell)},\forall k.
% % \end{equation}
% \begin{equation}\label{eq:cumulative attention matrix}
% T^{(k)} = 
% \begin{cases}    
%     \Gamma^{(k)} \prod\nolimits_{l = k_{max}}^{k_{max} - k + 1} \mathcal{A}^{(\ell)},
%     & \text{for FAGCN} \\
%     \Gamma^{(k)} \prod\nolimits_{l = 1}^k \mathcal{A}^{(\ell)},  & \text{for other models},
% \end{cases}
% \end{equation}
% where $T^{(0)} = \Gamma^{(0)}$.
% % \lucky{Note that although the formula for FAGCN appears different, it is equivalent at least in our theoretical analysis to the formula for the other models for any fixed value of $k_{max}$, since our theoretical analysis does not rely on the dependency between $\calA^{(k)}$'s and thus we can do variable substitution for the $\calA^{(k)}$'s to make the formula for FAGCN the same as the others.}
% The formula for FAGCN may appear different, but in our theoretical analysis, it is equivalent to the formula for other models when $k_{max}$ is fixed. This is because our theoretical analysis does not use the dependency between $\calA^{(k)}$'s, and thus we can do variable substitution to make the formula for FAGCN the same as the others.

\smallsection{Rephrased Propagation w.r.t $T^{(k)}$'s.}
Here, we discuss various representative attention-based GNNs (spec., GATv2, FAGCN, GPRGNN, and DAGNN).
We detail their attention functions in Table~\ref{tab:attention_functions}.
Those models are used throughout our theoretical analyses and empirical evaluation.

GATv2 and FAGCN learn edge attention $\alpha^{(k)}_{ij}$. GATv2 uses hidden features ($H_i \Vert H_j$), whereas FAGCN layer-aggregated features ($Z_i \Vert Z_j$), in computing each edge attention coefficient $\alpha^{(k)}_{ij}$. Notably, their $\alpha^{(k)}_{ij}$ have different bounds, such that GATv2's $\alpha^{(k)}_{ij} \in (0, 1)$ and FAGCN's $\alpha^{(k)}_{ij} \in (-1, 1)$. They do not learn hop attention coefficients, which can be expressed as a constant (1 for GATv2 and $c_{\gamma}$ for FAGCN).

%\footnote{The theoretical analysis can be trivially extended to the most GAT variants that computes row-wise stochastic $\mathcal{A}^{(k)}$}

%GATv2 concatenates the hidden features of each adjacent node pair ($H_i \Vert H_j$) with some transformations to compute the attention coefficients.
%Notably, the edge attention coefficients are normalized so that
%$\alpha^{(k)}_{ij} \in (0, 1)$ and $\sum_{j} \alpha^{(k)}_{ij} = 1, \forall i, j, k$.
%GATv2 does not learn hop attention, or equivalently, we can express GATv2's hop attention coefficients as constants, i.e., $\gamma_i^{(k)} \equiv 1, \forall i, k$.

%FAGCN concatenates the layer-aggregated features of adjacent node pairs ($Z_i \Vert Z_j$) with some transformations to compute the attention coefficients.
%Notably, $\operatorname{tanh}$ is applied when computing the pre-normalized edge attention coefficients, and thus,
%$\check{\alpha}^{(k)}_{ij} \in (-1, 1), \forall i, j, k$, after which degree normalization is used to obtain the (normalized) edge attention.
%FAGCN's hop attention coefficients are also constants:
%$\gamma_i^{(k)} \equiv c_{\gamma}, \forall i, k$, where $c_{\gamma}$ is a hyperparameter.

On the other hand, GPRGNN and DAGNN learn hop attention $\gamma_i^{(k)}$. GPRGNN's hop attention is not explicitly bounded and, thus, can learn negative hop attention $\gamma_i^{(k)}$. While $\gamma_i^{(k)} \in (0, 1)$ for DAGNN, it learns \textit{node-adaptive} hop attention.
Neither GPRGNN nor DAGNN learns nontrivial edge attention, and their edge attention coefficients are equivalently degree-normalized constants,
i.e., $\alpha^{(k)}_{ij} = 1 / \sqrt{d_i d_j}, \forall i,j,k$.

%GPRGNN uses a learnable variable for its hop attention.
%In each hop, this variable is identical for all the nodes.
%Specifically, for each $k$, $\gamma_i^{(k)} = \gamma_{j}^{(k)} = c_{k; \gamma}, \forall i, j$.
%DAGNN, unlike GPRGNN, learns \textit{node-adaptive} hop attention, where for each $i, k$,
%$H_i^{(k)}$, the $i$-th row of $H^{(k)}$, is used to compute $\gamma_i^{(k)}$.
%Neither GPRGNN nor DAGNN learns nontrivial edge attention, and their edge attention coefficients are equivalently degree-normalized constants,
%i.e., $\alpha^{(k)}_{ij} = 1 / \sqrt{d_i d_j}, \forall i,j,k$.


% GATv2, like most GAT variants, has row-wise stochastic edge attention matrices $\calA^{(k)}$'s, with each $\alpha_{ij}^{(k)}$ in $(0, 1)$.
% FAGCN's edge attention coefficients $\alpha_{ij}^{(k)}$'s are all in $(-1, 1)$.
% GPRGNN's hop attention coefficients $\gamma_i^{(k)}$'s are not explicitly bounded. 
% While for DAGNN, $\gamma_i^{(k)} \in (0, 1), \forall i, k$, only DAGNN has node-adpative $\gamma_i^{(k)}$.
The discussed GNNs consist of a representative and diverse set of attention functions, yet we can succinctly rephrase them w.r.t $T^{(k)}$ (see Table~\ref{tab: T}).\footnote{FAGCN and GATv2's propagation formulae are rewritten from their original form. Refer to Appendix~\ref{app:rewrite_msg_passing} for the details.}

==> icml2023/figures/S_T_.tex <==
\begin{figure}[htb]
    \centering   
    %\includegraphics[scale=0.35]{icml2023/fig/ST_and_performance/ST_and_performance_legend_230125a.pdf}\\ 
    \includegraphics[scale=0.35]{icml2023/fig/ST_and_performance/ST_and_performance_legend_230526.pdf}\\
    \begin{subfigure}[a]{\linewidth}
         \centering
         %\includegraphics[scale=0.35]{icml2023/fig/ST_and_performance/ST_combined_v0.pdf}\\
         \includegraphics[scale=0.28]{icml2023/fig/camera_ready_v/S(T).pdf}\\
         \vspace{-2mm}
         %\caption{}         
    \end{subfigure}
    \caption{\label{fig:S(T)_all}
    \bolden{The smoothness score $S(T^{(k)})$ of the cumulative attention matrix $T^{(k)}$ for each $k$.}
    \textit{\ours has (1) less smoothed $T^{(k)}$ over deep layers and
    (2) often un-smoothes $T^{(k)}$.}
    } 
%\vspace{3mm}
\end{figure}



==> icml2023/figures/S_T__v0.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.45\textwidth]{icml2023/fig/S(T).png}
    \includegraphics[scale=0.35]{icml2023/fig/ST/ST_legend_230123a.pdf}\\ 
    \includegraphics[scale=0.35]{icml2023/fig/ST/pubmed.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/ST/computer.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/ST/chameleon.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/ST/squirrel.pdf}
    \caption{\label{fig:flow_4} 
    % $S(T)$ at each layer $k$ over 64 layers. 
    \bolden{$S(T^{(k)})$ for each $k$ when $k_{max}=64$.}
    $\circ$ indicates a layer where $S(T^{(k)}) > S(T^{(k-1)})$, i.e., the attention matrix becomes less smooth. 
    Only \ours and FAGCN were able to unsmooth $T$, and $S(T)$ of \ours remains less smoothed over deep layers.
    % Circle marks indicate one of the layers where $S(T^{(k)}) > S(T^{(k-1)})$. 
    %The $x$-axis is in a log scale.
    %\fanchen{Claim.}
    %\fanchen{The circles seem not helpful in claiming that our model is good at making $T$ less smooth since there are more circles for FAGCN.}    
    } 
\end{figure}

==> icml2023/figures/Sum_T.tex <==
\begin{figure}[t]
    \centering    
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[scale=0.15]{icml2023/fig/sum_T/Sum_of_T(homophilic).pdf}
         \vspace{-2mm}
         \caption{}         
     \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[scale=0.15]{icml2023/fig/sum_T/Sum_of_T(heterophilic).pdf}
         \vspace{-2mm}
         \caption{}
     \end{subfigure}     
    \caption{\label{fig:sum_T}
    \bolden{Coefficients of the Sum of Cumulative Attention $(\sum_{l=0}^k T^{(l)})_{ij}$'s, when $k_{max}=64$.} 
    \textit{\ours always learns different importance for different node pairs even at deep layers.}
    }
\end{figure}



==> icml2023/figures/gamma_cv.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.45\textwidth]{icml2023/fig/Gamma_cv.png}
    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/gamma_legend_230123a.pdf}\\ 
    \includegraphics[scale=0.35]{icml2023/fig/cv_gamma/pubmed.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/cv_gamma/computer.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/cv_gamma/chameleon.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/cv_gamma/squirrel.pdf}
    
    \caption{\label{fig:flow_2} 
    \bolden{The coefficient of variation (CV) of $\gamma^{(k)}_i$'s for each $k$ with $k_{max}=64$.}
    %The $x$-axis is in a log scale.
    Only for \ours, the $\gamma^{(k)}_i$'s remain evidently node-varying over deep layers. 
    } 
\end{figure}

==> icml2023/figures/gamma_mean.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.45\textwidth]{icml2023/fig/Gamma_mean.png}

    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/gamma_legend_230123a.pdf}\\ 
    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/pubmed.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/computer.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/chameleon.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/mean_gamma/squirrel.pdf}
    
    \caption{\label{fig:flow_1} 
    \bolden{The mean value of $\gamma^{(k)}_i$'s for each $k$ with $k_{max}=64$.}
    %The $x$-axis is in a log scale.    
    The $\gamma^{(k)}_i$'s of \ours and GPRGNN are adaptive to graph homophily over deep layers.
    %but for GPRGNN, $S(T^{(k)})$ converges to $0$ as $k$ increases.
    }
\end{figure}

==> icml2023/figures/performance.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.45\textwidth]{icml2023/fig/Performance.png}

    \includegraphics[scale=0.35]{icml2023/fig/performance/performance_legend_230123a.pdf}\\ 
    \includegraphics[scale=0.35]{icml2023/fig/performance/pubmed.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/performance/computer.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/performance/chameleon.pdf}
    \includegraphics[scale=0.35]{icml2023/fig/performance/squirrel.pdf}
    
    \label{fig:flow_5} 
    \caption{
    % Model performance at . Star marks indicate the depth where each model achieved its best performance.         
    \textbf{The model performance at layers 2, 4, 8, 16, 32, and 64.}
    Each star symbol ($\filledstar$) indicates the best performance of each model.
    %The $x$-axis is in a log scale.    
    For \ours, the best performance is higher and achieved at a deeper layer overall.
    } 
\end{figure}

==> icml2023/tables/table-attention_function.tex <==
\begin{table*}[t]
\centering
\caption{Attention Functions of Graph Attention Models} \label{tab:attention_functions}
    \scalebox{0.90}{
    \renewcommand{\arraystretch}{1.0}
\begin{threeparttable}

%\vspace{0.5mm}
    \centering
    
    % \renewcommand{\arraystretch}{0.8}
        % \centering

        \begin{tabular}{c l l l}
            \toprule
            
            \multicolumn{1}{c}{Model} 
            & \multicolumn{1}{c}{Pre-normalized Edge Attention} 
            & \multicolumn{1}{c}{Normalized Edge Attention} 
            & \multicolumn{1}{c}{Hop Attention} 
            \\
            
            \midrule
            \midrule
            
            \textbf{GATv2}  & $ \check{\alpha}^{(k)}_{ij} = \exp((W^{(k)}_{edge})^{\top} \sigma (H_i^{(k-1)} \Vert H_j^{(k-1)})) $ 
                            & $ \alpha^{(k)}_{ij} = {\check{\alpha}^{(k)}_{ij}} / {\sum_{j' \in N(i)} \check{\alpha}^{(k)}_{ij'}} $
                            & $ \gamma^{(k)}_i = 1 $  
                        \\
            %\midrule
            % \vspace{0.5mm}
            
            \textbf{FAGCN}  & $ \check{\alpha}^{(k)}_{ij} = \tanh((W^{(k)}_{edge})^{\top} (Z_i^{(k-1)} \Vert Z_j^{(k-1)})) $ 
                            & $ \alpha^{(k)}_{ij} = {\check{\alpha}^{(k)}_{ij}} / {\sqrt{d_i d_j}}$
                            & $ \gamma^{(k)}_i = c_{\gamma}, \forall{k,i}$ (*)
                        \\
            %\midrule
            % \vspace{0.5mm}
            
            \textbf{GPRGNN} & $ \check{\alpha}^{(k)}_{ij} = 1 $ 
                            & $ \alpha^{(k)}_{ij} = {1} / {\sqrt{d_i d_j}}$
                            & $ \gamma^{(k)}_i = \gamma^{(k)}_j = c_{k; \gamma}, \forall k$ (**)
                        \\

            %\midrule
            % \vspace{0.5mm}
            
            \textbf{DAGNN}  & $ \check{\alpha}^{(k)}_{ij} = 1 $ 
                            & $ \alpha^{(k)}_{ij} = {1} / {\sqrt{d_i d_j}}$
                            & $ \gamma^{(k)}_i = \operatorname{sigmoid}( {W_{hop}}^{\top} H_i^{(k)} ) $ (***)
                        \\

            %\midrule
            
            %\textbf{\ours} & $ \check{\alpha}^{(k)}_{ij} = Softplus(W^{(k)}_{edge}^{\top} \sigma (Z_i^{(k-1)} \Vert Z_j^{(k-1)})) $ 
            %            & $ \alpha^{(k)}_{ij} = {\check{\alpha}^{(k)}_{ij}} / {\sqrt{\sum_{j' \in N(i)} \check{\alpha}^{(k)}_{ij'} \sum_{i' \in N(j)} \check{\alpha}^{(k)}_{ji'}}}$
            %            & $\gamma^{(k)}_i = ( {W_{hop}}^{\top} \sigma(H_i^{(k)} \Vert \tilde{Z}_i^{(k-1)} )) $  
            %            \\

            \bottomrule
        \end{tabular}        
        \begin{tablenotes}
        \small
        \item (*) for FAGCN, $c_\gamma$ is a hyperparameter fixed before training and is identical for all $k$ and $i$
        \item (**) for GPRGNN, $c_{k; \gamma}$ is a learnable variable that can be different for different $k$, but is identical for all $i$ given any fixed $k$
        \item (***) for DAGNN, the same $W_{hop}$ is used for each layer        
    \end{tablenotes}                
    % \vspace{-2mm}
\end{threeparttable}
}
\end{table*}

==> icml2023/tables/table-performance-AERO_non-linear_.tex <==

\begin{table*}[t]
\begin{center}
\caption{Node Classification Performance on Real-World Graphs} \label{tab:performance}
    \resizebox{\textwidth}{!}{
    \renewcommand{\arraystretch}{1.0}
        \centering
        \begin{tabular}{c c c c c c c c c c c c c }
            \toprule
            
            \textbf{Dataset} & Chameleon & Squirrel & Actor & Texas & Cornell & Wisconsin & Computer & Photo & Wiki-CS & Pubmed & Citeseer & Cora 
            \\

            \midrule
            
            \textbf{Homophily}  & 0.04 & 0.03 & 0.01 & 0.13 & 0.21 & 0.21 & 0.70 & 0.77 & 0.57 & 0.66 & 0.63 & 0.77 
            \\
            
            \midrule
            \midrule
            
            \midrule
            \textbf{\ours $^\ast$} & \textbf{71.58 $\pm$ 2.4} % chamleon
                            & \textbf{61.76 $\pm$ 2.4} % squir
                            & \textbf{36.57 $\pm$ 1.1} % actor
                            & \textbf{84.35 $\pm$ 5.2} % texas
                            & \textbf{81.24 $\pm$ 6.8} % cornell 
                            & \textbf{84.80 $\pm$ 3.3} % wisc
                            & \textbf{86.69 $\pm$ 1.4} % computer
                            & \textbf{92.50 $\pm$ 0.7} % photo
                            & \textbf{79.96 $\pm$ 0.5} % wiki 
                            & \textbf{80.65 $\pm$ 0.5} % pubmed
                            & \textbf{73.20 $\pm$ 0.6} % citeseer
                            & \textbf{84.02 $\pm$ 0.5} % cora
                         \\
                         
            \textbf{\ours $^\ast$} & 71.35 $\pm$ 1.8 % chamleon
                            & 61.31 $\pm$ 2.8 % squir
                            & 36.34 $\pm$ 0.9 % actor
                            & 84.00 $\pm$ 5.3 % texas
                            & 81.19 $\pm$ 6.4 % cornell 
                            & 83.57 $\pm$ 3.6 % wisc
                            & 84.75 $\pm$ 1.0 % computer
                            & 92.41 $\pm$ 0.6 % photo
                            & 79.89 $\pm$ 0.5 % wiki 
                            & 80.11 $\pm$ 0.7 % pubmed
                            & 72.98 $\pm$ 0.3 % citeseer
                            & 83.95 $\pm$ 0.6 % cora
                         \\
                         
            \textbf{\ours $^\ast$} & 71.58 $\pm$ 2.4 % chamleon
                            & 61.76 $\pm$ 2.4 % squir
                            & 36.57 $\pm$ 1.1 % actor
                            & 84.35 $\pm$ 5.2 % texas
                            & 81.24 $\pm$ 6.8 % cornell 
                            & 84.80 $\pm$ 3.3 % wisc
                            & 86.69 $\pm$ 1.4 % computer
                            & 92.50 $\pm$ 0.7 % photo
                            & 79.96 $\pm$ 0.5 % wiki 
                            & 80.65 $\pm$ 0.5 % pubmed
                            & 73.20 $\pm$ 0.6 % citeseer
                            & 84.02 $\pm$ 0.5 % cora
                         \\

            \bottomrule
        \end{tabular}
        }
    \begin{tablenotes}
      \scriptsize
      \item (*) In each column, \green{$\blacksquare$} indicates ranking the first, and \yellow{$\blacksquare$} indicates ranking the second. $\dag$ denotes the results borrowed from the original paper. (A.R. = average ranking) 
      \item (**) The number in each parenthesis () indicates the model's best performing layer for the given network. $\ast$ denotes the models with number of layers as a hyperparameter.
    \end{tablenotes}
\end{center}
\end{table*}

